REFINE: Enhancing Program Repair Agents through Context-Aware Patch Refinement

Large Language Models (LLMs) have recently shown strong potential in automatic program repair (APR), especially in repository-level settings where the goal is to generate patches based on natural language issue descriptions, large codebases, and regression tests. However, despite their promise, current LLM-based APR techniques often struggle to produce correct fixes due to limited understanding of code context and over-reliance on incomplete test suites. As a result, they frequently generate Draft Patches-partially correct patches that either incompletely address the bug or overfit to the test cases. In this work, we propose a novel patch refinement framework, Refine, that systematically transforms Draft Patches into correct ones. Refine addresses three key challenges: disambiguating vague issue and code context, diversifying patch candidates through test-time scaling, and aggregating partial fixes via an LLM-powered code review process. We implement Refine as a general refinement module that can be integrated into both open-agent-based and workflow-based APR systems. Our evaluation on the SWE-Bench Lite benchmark shows that Refine achieves state-of-the-art results among workflow-based approaches and approaches the best-known performance across all APR categories. Specifically, Refine boosts AutoCodeRover's performance by 14.67%, achieving a score of 51.67% and surpassing all prior baselines. On SWE-Bench Verified, Refine improves the resolution rate by 12.2%, and when integrated across multiple APR systems, it yields an average improvement of 14%-demonstrating its broad effectiveness and generalizability. These results highlight the effectiveness of refinement as a missing component in current APR pipelines and the potential of agentic collaboration in closing the gap between near-correct and correct patches. We also open source our code.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.14   Bib style update.  Documentation update.  DLT is now using
	       acmlarge format.
	       Generate error if a user tries to redefine sectioning commands

Version 2.13   Documentation update
	       Added mathcal in unicode mode
	       Bug fixes

Version 2.12   Bug fixes
	       Switched to unicode-math and libertinus for Unicode engines

Version 2.11   Conference date is no longer printed in bibstrip.
	       ISBN now uses 4-digit year
	       DOI in bibliography is now output as doi:XX.XXXX/XXXXX.XXXX
	       Changed URL in Creative Commons licenses (deleted
	       trailing /legalcode)

Version 2.10.  Bug fixes.  Documentation update.

Version 2.09.  Experimental tagging code is now in the main branch.
	       Creative Commons license is now allowed for all materials. 

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> samples/1_intro.tex <==

\section{Introduction}

% Large Language Models (LLMs) have demonstrated impressive capabilities in software engineering tasks such as code completion~\cite{chen2021evaluatinglargelanguagemodels}, test generation~\cite{10.1145/3643769, tufano2021unittestcasegeneration}, summarization~\cite{sun2024sourcecodesummarizationera}, and program repair~\cite{10.1145/3611643.3613892}. Building on these successes, recent benchmarks like SWE-Bench~\cite{jimenez2024swebenchlanguagemodelsresolve} have introduced the more realistic and challenging task of \emph{repository-level program repair}, where systems must generate patches that resolve user-submitted issues using information spread across large, multi-file codebases.

% Repository-level program repair represents a fundamental shift from traditional automated program repair, requiring systems to resolve complex, real-world software issues by synthesizing patches across extensive, multi-file codebases. Unlike conventional approaches that operate on isolated functions or small code fragments, this task demands understanding of intricate dependencies, cross-module interactions, and contextual relationships that span entire software repositories. Recent benchmarks such as SWE-Bench~\cite{jimenez2024swebenchlanguagemodelsresolve} have formalized this challenge, presenting systems with user-submitted issues that mirror the complexity encountered in production software development, where bug fixes often require coordinated changes across multiple files and deep comprehension of system architecture.


Large Language Models (LLMs) have made rapid progress on software engineering tasks such as code completion~\cite{chen2021evaluatinglargelanguagemodels}, test generation~\cite{10.1145/3643769, tufano2021unittestcasegeneration}, summarization~\cite{sun2024sourcecodesummarizationera}, and program repair~\cite{10.1145/3611643.3613892}. 
These successes have spurred a wave of research on applying LLMs to more realistic development scenarios—culminating in benchmarks like SWE-Bench~\cite{jimenez2024swebenchlanguagemodelsresolve}, which focuses on \emph{repository-level program repair} \CM{I think we do not need to highlight SWE-bench here, as it seems our appraoch is specific designed for SWE-bench, which is not the case}. 
Given a user-submitted issue, often expressend in natural language (NL), the goal is to produce a patch that resolves the bug without introducing regressions—reasoning over a large, multi-file codebase and validating correctness against comprehensive tests. \CM{I think the problem formulation here has some issues}


The community’s dominant response to repository-level repair has been agent-based: LLMs are treated as autonomous decision-makers equipped with tools—searching the codebase~\cite{wang2024openhands, yang2024sweagentagentcomputerinterfacesenable}, editing files~\cite{zhang2024autocoderover}, running tests~\cite{xia2024agentlessdemystifyingllmbasedsoftware}, and more. These agentic workflows aim to emulate how developers interact with their environment. Yet, this surge in tool-driven orchestration masks a deeper structural limitation: most agents operate at the level of \emph{surface control}—deciding which actions to take—but lack any real understanding of what the bug \emph{means}, what code \emph{matters}, or how to produce a \emph{coherent, generalizable} fix \CM{I think the limitation description is confusing}. As a result, they often generate brittle, hyper-local patches that overfit to test cases or misinterpret user intent.



In contrast, expert developers approach debugging \& repair as a hypothesis-driven, semantically grounded process~\cite{beller2017developers, nel2023crushingbugs}. Rather than immediately invoking tools, they begin by interpreting the issue report—reconstructing missing context, clarifying ambiguity, and forming hypotheses about the underlying problem. In practice, many developers rely on simple yet powerful techniques such as inserting print statements and examining execution logs to gain insight into the program’s behavior~\cite{beller2017developers}—often preferring these over more sophisticated debugging tool support. Through this inspection, they trace execution paths, analyze dynamic behavior, and reason about cross-file dependencies to identify the true root cause. Only then do they synthesize a patch—one that not only resolves the issue but also preserves architectural integrity and long-term maintainability. This workflow is intentional and semantically grounded—not a reactive sequence of tool invocations, but a structured process driven by understanding, reasoning, and design awareness.

To this end, we ask a simple but foundational question: \emph{What happens if we systematically introduce such semantic understanding of the issues and code into the decision points of an existing workflow-based agent?} Rather than building a monolithic, closed agent or defining a rigid pipeline, we explore how augmenting key stages of the repair workflow—with explicit representations of issue intent, runtime behavior, and code dependencies—impacts the quality of generated patches. Our system, {\ToolName}, embodies this hypothesis. It retains the modular structure and transparency of state-of-the-art workflow-based agent, AutoCodeRover~\cite{zhang2024autocoderover}~\rayb{or specrover?} \ap{I think AutoCodeRover is fine as I mentioned it more then SpecRover and mentioned it in the implementation section} \, but interleaves them with targeted reasoning modules that mirror how developers interpret, localize, and resolve issues. 

Specifically, we organize repository-level program repair into three  reasoning stages, each reflecting how developers approach real-world debugging. This structure enables a form of \emph{semantics-guided repair}, where LLM-based patch generation is scaffolded by structured reasoning about runtime behavior, issue intent, and code dependencies:




\begin{itemize}[leftmargin=1.5em]
    \item \textbf{Bug Localization via Execution Semantics}: Using program execution as a semantic signal, this stage aims to isolate the code regions most likely responsible for the reported failure.
    
    \item \textbf{Patch Refinement via Semantic Analysis}: This stage enhances a candidate patch using static reasoning over both the natural language issue and the program’s internal structure.
    \begin{itemize}
        \item \emph{Issue Semantics}: a structured representation of user intent extracted from the issue description;
        \item \emph{Code Semantics}: a model of code dependencies and control/data interactions affected by the patch.
    \end{itemize}

    \item \textbf{Reviewer-Inspired Patch Selection}: To mirror the deliberation step developers perform during code review, this final stage selects among competing patch candidates based on semantic alignment, completeness, and consistency.
\end{itemize}



% \ToolName{} instantiates this structure on top of existing agentic infrastructure~\cite{ruan2024specrovercodeintentextraction, zhang2024autocoderover}. The novel component includes reproducing the bug and collecting dynamic traces via test execution. 
% Next, the patch refinement agent takes in a base LLM-generated edit and enriches it using semantic signals. It parses the issue description into a structured intent representation and cross-checks the patch against program dependencies to eliminate inconsistencies or incomplete fixes. Finally, a reviewer-inspired aggregator agent ranks and selects the most semantically robust patch from a set of candidates. This layered approach allows \ToolName{} to move beyond surface-level edits and toward reasoning-driven, developer-aligned repairs.


\ToolName{} builds upon existing agentic infrastructures for program repair~\cite{ruan2024specrovercodeintentextraction, zhang2024autocoderover}, but introduces a modular reasoning layer that enables deeper semantic understanding. First, it reproduces the bug and collects execution traces by running the associated test suite—providing a runtime foundation for identifying fault-relevant regions in the code. The patch refinement agent then consumes an initial LLM-generated edit and systematically enriches it using semantic signals. It extracts a structured representation of the issue intent from natural language and analyzes program dependencies to ensure the proposed fix is both complete and contextually consistent. Finally, a reviewer-inspired aggregation agent evaluates candidate patches using these semantic criteria and selects the one best aligned with the inferred intent and overall program behavior. This layered architecture enables \ToolName{} to move beyond shallow, test-driven edits and toward reasoning-driven, developer-aligned repairs.




\rayb{update evaluation}

% List down the main contributions and the main results
To this end, we make the following contributions. 
%We believe this work will help future agents generate complete and consistent patches for repository-level repair.
\begin{enumerate}[leftmargin=*,noitemsep,topsep=0pt]

\item \textbf{\ToolName{}: A Semantics-Grounded Repair Pipeline.} We present \ToolName{}, a modular and semantics-aware repair pipeline that produces complete and consistent patches aligned with developer intent. \ToolName{} augments a workflow-based agent with three key reasoning components: (i) a bug localization agent grounded in execution semantics, (ii) a patch refinement agent incorporating both issue and code semantics, and (iii) a reviewer-inspired aggregation module that selects the most coherent patch among candidates.

\item \textbf{Semantic Foundations for Reasoning-Driven Repair.} We integrate both dynamic and static semantic signals to guide each stage of the repair process. For localization, we leverage \emph{execution semantics}—including test-driven failure reproduction and dynamic trace analysis—to accurately isolate fault-relevant regions, outperforming retrieval-based baselines. For patch refinement, we introduce two complementary forms of static semantics: \emph{issue semantics}, which captures user intent from natural language, and \emph{code semantics}, which encodes dependency-aware program structure. Through targeted ablation studies, we demonstrate that these semantic components are critical for producing generalizable, consistent, and developer-aligned patches.


\item \textit{Evaluation.} \ToolName{} scores 44.66\% on SWE-Bench Lite, the highest among workflow-based methods. With full semantic integration in a multi-agent setup, it shows the potential of achieving around 51.33\%—leading the leaderboard across workflow-based and open-process agentic methods, with only a learning-based agent (a different category) ahead.~\rayb{update}
\end{enumerate}




We hope that future works incorporate elements of our approach into their pipeline by leveraging semantics-aware reasoning to resolve repository-level issues. In what follows, we discuss important related work (\S\ref{sec:related_work}), motivate our methodology with the help of an example (\S\ref{sec:motivation}), explain our specific methodology (\S\ref{sec:methodology}), and report our experimental results on SWE-Bench Lite (\S\ref{sec:experiments}). We also provide the prompts used in (\S\ref{sec:prompts_used}).

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{motivational-example-new.pdf}
    \caption[]{Motivating Example - \blackcircled{1} is the issue description, \blackcircled{2} is the developer patch \& SemAgent patch, \blackcircled{3} and \blackcircled{4} are incomplete/overfitted patches \CM{I did not know the definition of incomplete/overfitted patches here}, \blackcircled{5} is the \ToolName{} generated issue semantics, \blackcircled{6} is the \ToolName{} generated code semantics.
    %~\ray{I think 3 is incomplete, not inconsistent----changing the text}
    }
    \label{fig:motivating}
\end{figure*}



==> samples/backup/1_into.v0.tex <==

\section{Introduction}




% What is the problem? -- program level respository repair
%Recent emergent capabilities of 
In recent years, LLMs have shown remarkable progress in self-contained, short context software engineering tasks such as function completion \cite{chen2021evaluatinglargelanguagemodels}, test case generation \cite{10.1145/3643769, tufano2021unittestcasegeneration}, function summarization \cite{sun2024sourcecodesummarizationera}, and bug resolution \cite{10.1145/3611643.3613892}. Given this success, recent works such as SWE-Bench \cite{jimenez2024swebenchlanguagemodelsresolve} have introduced challenging software engineering benchmarks requiring LLMs to reason at larger repository-level contexts. In particular, these benchmarks introduce the task of {repository-level program repair}. SWE-Bench curates such program repair tasks from resolved user-submitted issues in open-source repositories. Each repair task has three components: (i) a natural language user issue, (ii) a ground-truth developer patch, and (iii) test cases that reliably measure the efficacy of a patch. 

% Why is it interesting / important / hard ? --
Repository-level program repair poses unique challenges for LLMs: (a) accurately interpreting the user-reported issue, (b) retrieving and reasoning over relevant code context—including dependencies across multiple functions and files, and (c) generating patches that meet the standards of expert developers by resolving the issue without breaking existing functionality. Advancing this task is essential for reducing developer burden and accelerating issue resolution. As a result, the task has attracted growing interest from both academia~\cite{zhang2024autocoderoverautonomousprogramimprovement, ruan2024specrovercodeintentextraction, xia2024agentlessdemystifyingllmbasedsoftware, wang2025openhandsopenplatformai, yang2024sweagentagentcomputerinterfacesenable} and industry~\cite{AWSAmazonQDeveloper, Cognition}, particularly through the development of agentic solutions.


% The problem of repository-level program repair is unique as it requires LLMs to (a) develop an accurate understanding of the given user issue, (b) retrieve relevant code context and comprehend intricate dependencies spanning multiple functions within a module and possibly multiple files in a repository, and (c) generate patches that adhere to the strict standards of expert human developers - successfully resolving the given issue while simultaneously retaining existing functionality. Progress on repository-level program repair is crucially important as it can help alleviate developer fatigue and improve issue fixing velocity. As a result, this area of research has attracted significant attention both from academia \cite{zhang2024autocoderoverautonomousprogramimprovement, ruan2024specrovercodeintentextraction, xia2024agentlessdemystifyingllmbasedsoftware, wang2025openhandsopenplatformai, yang2024sweagentagentcomputerinterfacesenable}, and industry \cite{AWSAmazonQDeveloper, Cognition}. 

% Why hasn't it been solved before? OR what's wrong with previous proposed solutions? What is the key problem you have identified ?
Existing repository-level program repair methods fall into two main categories: open-process agent-based and workflow-based~\cite{anthropic}. \textit{Agent-based} methods treat LLMs as completely autonomous agents -- equipping them with tools to interact within a pre-defined environment.  While effective~\cite{wang2025openhandsopenplatformai, yang2024sweagentagentcomputerinterfacesenable, Cognition}, they often suffer from non-deterministic behavior, limited transparency, and poor controllability—making them difficult to trust, reproduce, or integrate into structured development workflows. \CM{There are two issues here (1) why they are suffering the non-deterministic limitation? we should explian the ration here  (2)do we have reproducibility/deterministic evaluation to support our advantage?}




% Existing research works that attempt to solve this problem primarily fall into two categories: open-process agent-based and  workflow-based~\cite{anthropic}. \textit{Agent-based} methods treat LLMs as completely autonomous agents -- equipping them with tools to interact within a pre-defined environment. While such techniques \cite{wang2025openhandsopenplatformai, yang2024sweagentagentcomputerinterfacesenable, Cognition} have demonstrated relatively good performance, they often suffer from the unpredictable and erratic nature of arbitrary decision making. As a result, it is difficult for users of this approach to exercise control or expect consistency when using such techniques.

\textit{Workflow-based} approaches ~\cite{zhang2024autocoderoverautonomousprogramimprovement, ruan2024specrovercodeintentextraction, xia2024agentlessdemystifyingllmbasedsoftware}, on the other hand, propose guiding LLMs through pre-defined, task-specific procedures for repository-level program repair. These approaches leverage specialized tooling and exhibit greater determinism compared to open-ended, agent-based methods. While effective in addressing the primary issue, we observe that they often produce \textit{hyper-localized} patches — either 
(a) overfitting to specific bug-producing examples in the user's issue description, or (b) resolving the main issue but overlooking edge cases or broader consistency requirements. \CM{we should refer to our data for these two limitations, and expalin more here}
This limitation arises from two key challenges: (i) insufficient semantic understanding of the user issue and its associated code dependencies, and (ii) limited use of available execution semantics.


% \textit{Workflow-based} approaches \cite{zhang2024autocoderoverautonomousprogramimprovement,ruan2024specrovercodeintentextraction, xia2024agentlessdemystifyingllmbasedsoftware}, on the other hand, force LLMs to follow a pre-defined procedure specially designed for the task of repository-level program repair. These methods often rely on tooling specifically designed for the problem at hand and are more deterministic than agent-based approaches. While these methods are very effective at repository-level program repair, we find that such methods often generate patches that hyper-localize to the user-given issue, generating patches that (a) either over-fit to specific user-provided examples~\ray{where in the workflow use example is provided?} or (b) resolve the bulk of the given issue but miss out on code edits needed to cover edge cases or keep the codebase consistent. We note that this primarily stems from (i) the lack of a deep semantic understanding of the user issue and the related intricate code dependencies or (ii) the under-leveraging of available execution semantics.

% How does your approach differ ? What are the benefits ? What are the limitations ? What are the main components of your approach ?
\textbf{Our work.}  To address the limitations of existing approaches, we propose \ToolName{}—a \textit{semantics-aware}, workflow-based technique that produces patches which are both \textit{complete} and \textit{consistent}. While retaining the reliability of workflow-based methods, \ToolName{} achieves superior performance by deeply understanding the user issue, code implementation, and execution behavior. \ToolName{} consists of two key components:

\begin{itemize}[leftmargin=*,noitemsep,topsep=0pt]
    \item \textbf{Bug Localization via Execution Semantics}: This component leverages a suite of methods—including issue reproduction, execution trace analysis, and spectrum-based fault localization—to identify buggy code regions relevant to the reported issue.
    
    \item \textbf{Patch Refinement via Semantic Analysis}: Given a candidate patch (often incomplete or inconsistent), this component refines it using:
    \begin{itemize}[leftmargin=*,noitemsep,topsep=0pt]
        \item \textbf{Issue Semantics}, which extracts intent and context from the user-reported issue. (issue -> (buggy file information?))
        \item \textbf{Code Semantics}, which captures and reasons about underlying code dependencies affected by the patch.
    \end{itemize}
\end{itemize}
\CM{here, we define many semantics, but the definitions are ambiguous, we need to put a formal and percise definition of each semantic (via mathmatical equation or examples) in our motivation section}

Together, these components enable \ToolName{} to generate high-quality fixes grounded in semantic understanding.



%To mitigate the above mentioned problems, we propose \ToolName{} - a code \textit{semantics-aware} workflow-based technique that can generate patches that are both \textit{complete} and \textit{consistent}. Thus, while our approach enjoys the consistent nature of workflow-based methods, it can achieve superior performance by leveraging a deep semantic understanding of the user issue, code implementation, and execution information.  To do so, we design \ToolName{} to have two main components. The first is a component that leverages execution semantics through a consortium of methods, including issue reproduction, execution trace analysis, and spectrum-based fault localization. \ToolName{} uses these semantics to localize buggy context relevant to the user issue. The second is a patch-refinement step that takes in a candidate patch (often \textit{incomplete} or \textit{inconsistent}) and refines the patch by leveraging two sub-components - an issue-semantics component that distills understanding from the user-provided issue and a code-semantics component that explicitly understands the intricate code dependencies affected by the candidate patch.    

% List down the main contributions and the main results
To this end, we make the following contributions. 
%We believe this work will help future agents generate complete and consistent patches for repository-level repair.
\begin{enumerate}[leftmargin=*,noitemsep,topsep=0pt]

\item \textit{\ToolName{}} - We introduce \ToolName{}, a novel pipeline that excels at creating complete patches that align with developer expectations. \ToolName{} pipeline consists of an improved bug localization agent with execution semantics, a novel patch repair agent (with issue and code semantics), and new patch reviewing and aggregator agents.
%We evaluate our methodology on SWE-Bench Lite and achieve a remarkable performance of $43.33\%$, placing us second on the open-source leaderboard and the first among open-source techniques that do not require any explicit fine-tuning.

\item \textit{Issue Semantics and Program Semantics} - We highlight the importance for agents to develop a deeper understanding of code semantics (both issue and underlying program semantics). We validate the need for such semantics through extensive ablations.

\item \textit{Execution Semantics} - We showcase the utility of using execution semantics for the accurate localization of buggy context for the relevant issue. % at hand.

\item \textit{Evaluation.} \ToolName{} scores 44.66\% on SWE-Bench Lite, the highest among workflow-based methods. With full semantic integration in a multi-agent setup, it shows the potential of achieving around 51.33\%—leading the leaderboard across workflow-based and open-process agentic methods, with only a learning-based agent (a different category) ahead.
\end{enumerate}

%We evaluate \ToolName{} on SWE-Bench Lite benchmark and achieve SOTA performance of $43.33\%$ among all the workflow-based models. While combining the semantics from all the related sources, we show the potential of reaching up to 50\%  (top on the SWE-Bench Lite leader-board across all open process agentic and workflow based approaches). 

We hope that future works incorporate elements of our approach into their pipeline by leveraging semantics-aware reasoning to resolve repository-level issues. In what follows, we discuss important related work (\S\ref{sec:related_work}), motivate our methodology with the help of an example (\S\ref{sec:motivation}), explain our specific methodology (\S\ref{sec:methodology}), and report our experimental results on SWE-Bench Lite (\S\ref{sec:experiments}). We also provide the prompts used in (\S\ref{sec:prompts_used}).

% What are the key components of my approach and results? Also include any specific limitations.
% To enable 

% Then have a final paragraph or subsection: "Summary of Contributions". It should list the major contributions in bullet form, mentioning in which sections they can be found


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.8\linewidth]{Images/simple-overview.pdf}
%     \caption[]{Patch Repair procedure augmented by \ToolName{} (blue boxes) and a traditional APR Agent (green boxes)}
%     \label{fig:simple-overview}
% \end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{motivational-example-new.pdf}
    \caption[]{Motivating Example - \blackcircled{1} is the issue description, \blackcircled{2} is the developer patch \& SemAgent patch, \blackcircled{3} and \blackcircled{4} are incomplete/overfitted patches, \blackcircled{5} is the \ToolName{} generated issue semantics, \blackcircled{6} is the \ToolName{} generated code semantics.
    %~\ray{I think 3 is incomplete, not inconsistent----changing the text}
    }
    \label{fig:motivating}
\end{figure*}



==> samples/backup/4_method.v1.tex <==
\begin{figure*}[pt]
    \centering
    %\includegraphics[width=0.8\textwidth]{Images/overview-Overall_Workflow_biggerletters.drawio.pdf}
    \includegraphics[width=\textwidth]{SemAgent_Overall.png}
    \caption[]{\textbf{Pipeline of \ToolName{}}. {\small It takes as input a \textit{codebase}, \textit{GitHub issue}, and \textit{regression tests}.
    First, it uses \textit{execution semantics} \circled{1} to localize the buggy code \circled{2} and apply a standard APR workflow—patch generation \circled{3}, validation \circled{4}, and selection \circled{5}—producing a candidate patch, which is often incomplete or inconsistent. Next, \ToolName{} refines this patch using issue \circled{6} and code semantics \circled{8}, extracted from the buggy file \circled{7} and candidate patch \circled{5}. 
    This yields fine-grained fixes \circled{10}, which a reviewer agent \circled{11} filters based on the issue, selecting relevant edits \circled{12}. These are aggregated with the candidate patch \circled{13} and refined using execution feedback \circled{14} to produce the final patch \circled{15}. All the semantic components are highlighted with dashed boxes.}}
    \label{fig:pipeline}
\end{figure*}


\section{Methodology}
\label{sec:methodology}

% start with the maths equations setting up the problem and what functions we are actually implementing

% explain componenets in detail
\subsection{Problem Formulation}


%In repository-level code repair, given a Python codebase \(\mathcal{D}\) with regression tests \(\mathcal{T}\) and an issue statement \(\mathcal{I}\), the objective is to generate a patch \(p\) such that the updated codebase \(\mathcal{D}'\) (after applying \(p\)) passes an augmented test suite \(\mathcal{T}'\), which includes new or modified tests that reproduce the issue. However, initial patches produced by repository-level repair may be over-fitted to the test case or incomplete---resolving only part of the issue or introducing regressions. Our objective is to detect and refine such partially correct patches to produce a correct patch that ensures \(\mathcal{D}'\) passes \(\mathcal{T}'\), thereby confirming both issue resolution and preservation of original functionality.


% We formally define \ToolName{} as a function \(\mathcal{F}(\mathcal{I}, \mathcal{D}, \mathcal{T}) \rightarrow p\), which generates the final patch $p$. First, \ToolName{} follows a standard Automated Program Repair (APR) pipeline--bug localization, patch generation, validation, and selection--to produce an initial patch \(p_{\text{ini}}\), which may be partial or incorrect. 
% In this step, \ToolName{} provides semantics of code execution \((\mathcal{E})\) to facilitate this process.
% To refine it, the repair module \(R\) takes \(p_{\text{ini}}\), the original codebase \(\mathcal{D}\), issue semantics \(\mathcal{I}'\) (computed via semantic analysis \(G(\mathcal{I}) \rightarrow \mathcal{I}'\)), and code semantics \(\mathcal{C}'\) (computed via semantic analysis \(S(\mathcal{C}) \rightarrow \mathcal{C}'\)) \CM{ whats is  $C$ here is unknown}, and generates a set of candidate patches \(\mathcal{P}' = \{p'_1, p'_2, \dots\}\).


We define \ToolName{} as a two-stage patch generation system that incrementally refines an initial patch toward a final, correct repair. Given an issue statement \(\mathcal{I}\), a Python codebase \(\mathcal{D}\), and a regression test suite \(\mathcal{T}\), the objective is to generate a patch \(p\) such that the updated codebase \(\mathcal{D}'\) passes an augmented test suite \(\mathcal{T}'\), which includes additional tests that reproduce the issue described in \(\mathcal{I}\). This process can be defined as: $\mathcal{F}(\mathcal{I}, \mathcal{D}, \mathcal{T}) \rightarrow p$, 
where, \(\mathcal{F}\) is implemented as a pipeline of the following stages:

\paragraph{Stage 1: Initial Patch Generation}

\ToolName{} first generates an initial patch:
\[
p_{\text{init}} = \mathcal{F}_{\text{init}}(\mathcal{I}, \mathcal{D}, \mathcal{T}),
\]
using a standard Automated Program Repair (APR) pipeline that includes bug localization, patch generation, validation, and selection. The resulting patch \(p_{\text{init}}\) is often incomplete or overfitted—it may fix specific symptoms without generalizing to all failure contexts, or it may introduce regressions.

\paragraph{Stage 2: Patch Refinement via Contextual Reasoning}

To refine \(p_{\text{init}}\), \ToolName{} constructs two forms of context based on both the issue and the patched code:

\begin{itemize}[leftmargin=*]
    \item \textbf{Issue context:} \(\mathcal{I}' = \mathcal{G}(\mathcal{I}, \mathcal{D})\), computed by grounding the natural language issue statement \(\mathcal{I}\) in the structure and behavior of the codebase \(\mathcal{D}\). This may include extracting relevant call paths, stack traces, involved files and functions, and test artifacts that reproduce the failure.
    
    \item \textbf{Code context:} \(\mathcal{C}' = \mathcal{S}(\mathcal{D}, p_{\text{init}})\), capturing how the initial patch interacts with  \(\mathcal{D}\), including call graph, data flow, control flow, and runtime side effects.
\end{itemize}

Using these contexts, the refinement module generates a set of refined candidate patches:
\[
\mathcal{P}' = \mathcal{R}(\mathcal{D}, p_{\text{init}}, \mathcal{I}', \mathcal{C}').
\]
Each \(p'_i \in \mathcal{P}'\) is an incremental modification of the initial patch \(p_{\text{init}}\), aimed at resolving semantic gaps and aligning the behavior of the codebase with the intended fix.

\paragraph{Stage 3: Final Selection}

Finally, \ToolName{} selects the best candidate patch using a test-based selection mechanism:
\[
p = \textsc{Select}(\mathcal{P}', \mathcal{T}'),
\]
where \(\mathcal{T}'\) is the augmented test suite that includes \(\mathcal{T}\) and any newly synthesized or modified tests that validate the issue resolution. The selected patch \(p\) ensures that the issue is resolved while preserving the original functionality, as verified by \(\mathcal{T}'\).


We generate many such candidate patches and pass it to a code reviewing agent \(\mathcal{V}\) that selects a subset \(\mathcal{P}''\) $\subseteq$ \(\mathcal{P}'\) of patches that are filtered based on relevancy in resolving the issue. From this subset, the final patch $p$ is constructed by combining the incomplete patch $p_{ini}$ and \(\mathcal{P}''\) and passing it through a patch generation agent that performs a final aggregation along with refinement and validation. 

Figure \ref{fig:pipeline} shows the complete outline of \ToolName{}. In the rest of the section we will elaborate design and implementation of each of these components. 

% Our contributions are three-fold: (1) we design the repair stage, (2) formulate semantics of code, execution, and issues, and (3) implement a patch reviewer agent. We also show how these semantics enhance patch correctness, consistency, and context localization. Figure \ref{fig:pipeline} shows the complete outline of \ToolName{}.

\begin{comment}


\subsubsection{Issue Context}



{Issue Context} is a structured, implementation-agnostic representation that captures the relevant intent, scope, and behavioral expectations underlying a reported software issue. It transforms unstructured natural language descriptions into actionable guidance for reasoning about and constructing a valid repair.


We represent an issue context \( I \) as a 5-tuple:
\[
I = (T, L, A, C, G)
\]
where:
\begin{itemize}[leftmargin=1.5em]
    \item \( T \): \textbf{Target} — System components implicated by the issue.
    \item \( L \): \textbf{Logic} — The intended change in system behavior.
    \item \( A \): \textbf{Actions} — High-level plans required to realize the change.
    \item \( C \): \textbf{Constraints} — Conditions that must be preserved post-fix.
    \item \( G \): \textbf{Generalization} — The scope of applicability beyond the specific instance.
\end{itemize}

For the issue described in Figure~\ref{fig:motivating}, the corresponding issue context is as follows: the \textbf{target} (\(T\)) is the QDP parser's command matching logic; the \textbf{logic} (\(L\)) involves transforming case-sensitive command recognition into case-insensitive behavior; the \textbf{actions} (\(A\)) include identifying all locations where command strings are compared and updating them to use case-insensitive methods (e.g., normalization or tolerant matching); the \textbf{constraints} (\(C\)) require preserving the parser's existing behavior for uppercase inputs and avoiding crashes on lowercase inputs; and the \textbf{generalization} (\(G\)) specifies that the fix should apply to all QDP commands, not just the specific instance of \texttt{READ SERR}.

The issue context serves as an intermediate reasoning layer between informal user-reported bugs and code-level repair actions, enabling structured understanding and guiding patch generation in a semantically meaningful way.




\subsubsection{Patch Context}





\textbf{Patch Context} is a structured representation of the semantic environment surrounding a candidate patch. It captures the relevant data dependencies, control structure, behavioral constraints, and dynamic call relationships that determine how the patch interacts with its surroundings.
%whether a patch is locally correct and safely integrable into the broader program.


We define the patch context \( \mathcal{C}(P) \) for a patch \( P \) at location \( \ell \) as:
\[
\mathcal{C}(P) = (\mathsf{DD}_\ell, \mathsf{CD}_\ell, \mathsf{IC}_\ell, \mathsf{CG}_\ell)
\]
where:
\begin{itemize}[leftmargin=1.5em]
    \item \( \mathsf{DD}_\ell \): \textbf{Data Dependencies} — Variables and expressions read/written at \( \ell \), including transitive flows (e.g., line content, regex matches).
    \item \( \mathsf{CD}_\ell \): \textbf{Control Dependencies} — Control-flow constructs affecting the execution of \( \ell \), such as conditional branches and loops.
    \item \( \mathsf{IC}_\ell \): \textbf{Invariant Constraints} — Semantic assumptions and correctness conditions that must be preserved before and after the patch (e.g., input format validity, crash avoidance).
    \item \( \mathsf{CG}_\ell \): \textbf{Call Graph Context} — A backward-traceable call chain showing which higher-level components transitively reach \( \ell \), capturing its functional embedding in the system.
\end{itemize}

For example, in the QDP parser issue described in Figure~\ref{fig:motivating}, the candidate patch modifies the `\_line\_type' function responsible for identifying command lines. The data dependencies include the regular expression `\_command\_re', which encodes the expected command syntax, and the input lines being matched against it. The control dependencies span the call chain from `Table.read', through `QDP.read', etc. % `_read_table_qdp`, `_get_tables_from_qdp_file`, and `_get_type_from_list_of_lines`, down to `_line_type`. 
The invariant constraints require that lowercase commands such as \texttt{read serr 1 2} be recognized as valid without breaking compatibility with existing uppercase-only behavior, and without introducing regressions or crashes elsewhere in the parsing process.

The patch context serves as a semantic scaffold for reasoning about the correctness and consistency of candidate patches, enabling principled refinement and post-hoc validation of learned edits.

\end{comment}


% \subsection{Execution Semantics for Bug Localization}

% The execution semantics module (\circled{1} in Figure \ref{fig:pipeline}) localizes bugs by triangulating evidence from three sources: (1) crash reports from reproducers, providing coarse failure signals; (2) execution traces identifying actively involved files; and (3) Spectrum-Based Fault Localization~\cite{abreu2007accuracy}, which statistically ranks file suspiciousness using test outcomes. The localized regions are passed to an APR workflow (\circled{2} to \circled{5} in Figure \ref{fig:pipeline}) to generate an initial patch, which is then refined in \ToolName{}'s repair stage. 
\subsection{Stage 1: Initial Patch Generation}

\subsection{Stage 2: Patch Refinement}
The goal of this stage is to refine an incomplete patch (\circled{5}) by generating a set of fine-grained fixes (\circled{10}) that resolve many incomplete patches and address the underlying issue. This stage comprises of three components:
\begin{enumerate}[label={\alph*.}]
    \item Extracting issue context  (\circled{6});
    \item Extracting relevant code context (\circled{8});
    \item generating potential patches using the above two. % both (\circled{9}, \circled{10})
\end{enumerate}

% (1) extracting issue semantics from the issue description (\circled{6}), (2) leveraging these to infer code semantics (\circled{8}), and (3) generating fixes using both (\circled{9}, \circled{10}).
\noindent
\subsubsection{Extracting Issue Context.} 
GitHub issues often include natural language descriptions, examples, and reproduction steps, but LLMs may overfit to specific instances (e.g., block \blackcircled{4} in Figure~\ref{fig:motivating}) or fail to generalize from under-specified inputs. To mitigate this, we compute the \emph{issue context} \(\mathcal{I}' = \mathcal{G}(\mathcal{I}, \mathcal{D})\) by grounding the issue statement \(\mathcal{I}\) in the structure and behavior of the codebase \(\mathcal{D}\). This gives us a structured abstraction that captures the relevant intent, scope, and behavioral expectations underlying a reported software issue. It transforms unstructured natural language into actionable guidance for reasoning about and constructing valid repairs.

Formally, we represent an issue context \(I\) as a 5-tuple: $I = (T, L, A, C, G)$, where:
\begin{itemize}[leftmargin=1.5em]
    \item \( T \): {Target} — The system components implicated by the issue.
    \item \( L \): {Logic} — The intended change in system behavior.
    \item \( A \): {Actions} — High-level plans required to realize the change.
    \item \( C \): {Constraints} — Conditions that must be preserved after the fix.
    \item \( G \): {Generalization} — The scope of applicability beyond the specific instance.
\end{itemize}

For the issue illustrated in Figure~\ref{fig:motivating}, the corresponding issue context is as follows: the \textbf{target} (\(T\)) is the QDP parser’s command matching logic; the \textbf{logic} (\(L\)) involves transforming case-sensitive command recognition into case-insensitive behavior; the \textbf{actions} (\(A\)) include identifying all locations where command strings are compared and updating them to use case-insensitive methods (e.g., normalization or tolerant matching); the \textbf{constraints} (\(C\)) require preserving the parser’s existing behavior for uppercase inputs and avoiding crashes on lowercase inputs; and the \textbf{generalization} (\(G\)) specifies that the fix should apply to all QDP commands, not just the specific instance of \texttt{READ SERR}.

The issue context acts as an intermediate reasoning layer between informal user-reported issues and concrete code-level repair actions. By providing a structured abstraction over the problem space, it guides patch generation in a semantically meaningful and generalizable manner.

% \textbf{Extracting Issue Context.} GitHub issues often include detailed descriptions, examples, and reproduction steps. Thus, LLMs often overfit to some specific example/steps (e.g., block \blackcircled{4} in Figure~\ref{fig:motivating}) or struggle with under-specified descriptions—both common in SWEBench Lite. To address this, we design an agent to extract issue context %introduce a prompting step that guides the LLM 
% to abstract beyond surface artifacts and produce structured semantic directions reflecting the core intent of the issue. These high-level signals ground the repair process, improving generalization and alignment with developer expectations.

% To this end we define {\em Issue Context} as a structured, implementation-agnostic representation that captures the relevant intent, scope, and behavioral expectations underlying a reported software issue. It transforms unstructured natural language descriptions into actionable guidance for reasoning about and constructing a valid repair.


% We represent an issue context \( I \) as a 5-tuple:
% \[
% I = (T, L, A, C, G)
% \]
% where:
% \begin{itemize}[leftmargin=1.5em]
%     \item \( T \): {Target} — System components implicated by the issue.
%     \item \( L \): {Logic} — The intended change in system behavior.
%     \item \( A \): {Actions} — High-level plans required to realize the change.
%     \item \( C \): {Constraints} — Conditions that must be preserved post-fix.
%     \item \( G \): {Generalization} — The scope of applicability beyond the specific instance.
% \end{itemize}

% For the issue described in Figure~\ref{fig:motivating}, the corresponding issue context is as follows: the \textbf{target} (\(T\)) is the QDP parser's command matching logic; the \textbf{logic} (\(L\)) involves transforming case-sensitive command recognition into case-insensitive behavior; the \textbf{actions} (\(A\)) include identifying all locations where command strings are compared and updating them to use case-insensitive methods (e.g., normalization or tolerant matching); the \textbf{constraints} (\(C\)) require preserving the parser's existing behavior for uppercase inputs and avoiding crashes on lowercase inputs; and the \textbf{generalization} (\(G\)) specifies that the fix should apply to all QDP commands, not just the specific instance of \texttt{READ SERR}.

% The issue context serves as an intermediate reasoning layer between informal user-reported issues and code-level repair actions, enabling structured understanding and guiding patch generation in a semantically meaningful way.



% the goal of this stage is to take in a potentially incomplete patch \circled{5} and generate a set of Fine-grained Fixes \circled{10} that fix inconsistencies and help the patch resolve the issue. The repair stage can be broken into 3 main components: Generating the issue semantics \circled{6} from the issue description, leveraging this to understand code semantics \circled{8} and finally using this information in a Fix generation stage \circled{9} that generates the final fixes \circled{10}.

% \textbf{Generating Issue Semantics.} Software issues, such as those commonly found on GitHub and in our motivating example \blackcircled{1}, usually start with an issue description, followed by examples with the expected and actual results along with reproduction steps and system information. While rich in detail, such descriptions can lead large language models (LLMs) to overfit on specific artifacts such as the examples as seen in the over-fitted patch \blackcircled{4} during downstream automated program repair (APR) tasks. Moreover, under-specified issue description which are a frequent occurrence in SWEBench Lite—pose additional challenges, often resulting in incorrect or incomplete fixes.

% To address these limitations, we introduce a dedicated prompting step that encourages the LLM to reason beyond surface-level artifacts. The LLM is prompted to identify whether the issue represents a broader class of problems and to generate structured semantic directions that capture the underlying intent of the issue. These directions serve as high-level guidance for the rest of the repair workflow, enabling it to generalize better and resolve issues more reliably. This semantic grounding is a critical step for consistent and developer-aligned patch generation. 

\noindent
\subsubsection{Extracting relevant code context}
%\textbf{Generation of Code Semantics.} 
To generate robust patches, it is not enough to understand the issue alone—\ToolName{} must also capture how the code behaves in relation to the issue and the proposed fix. We define the \emph{code context} as \(\mathcal{C}' = \mathcal{S}(\mathcal{D}, p_{\text{init}})\), which models the interaction between the initial patch and the codebase \(\mathcal{D}\), including call graphs, data flow, control flow, and runtime side effects. This step builds a understanding of code intent, usage, and its relevance to the bug.

% In particular, we extract high-level execution flows that connect the issue to the affected program behavior. These flows represent meaningful control and data pathways that are candidates for localized repair. In our motivating example, we identify four such flows (\blackcircled{6}), including reading a QDP table, processing QDP lines, writing QDP tables, and regex operations.

% \textit{Step-Level Reasoning.} Each execution flow is decomposed into fine-grained, natural language steps (e.g., “read file line by line”, “extract header row”) that align with how developers reason about behavior. To map these steps back to code, we prompt an LLM with step descriptions and relevant file content. The model produces structured JSON outputs mapping semantic roles to concrete code snippets, enabling precise and context-aware localization for refinement.

To this end, we define \textbf{Patch Context} as a structured representation of the semantic environment surrounding a candidate patch. It captures the relevant data dependencies, control structure, behavioral constraints, and dynamic call relationships that determine how the patch interacts with its surroundings.
%whether a patch is locally correct and safely integrable into the broader program.


We define the patch context \( \mathcal{C}(P) \) for a patch \( P \) at location \( \ell \) as:
$\mathcal{C}(P) = (\mathsf{DD}_\ell, \mathsf{CD}_\ell, \mathsf{IC}_\ell, \mathsf{CG}_\ell)$, where :
\begin{itemize}[leftmargin=1.5em]
    \item \( \mathsf{DD}_\ell \): \textbf{Data Dependencies} — Variables and expressions read/written at \( \ell \), including transitive flows (e.g., line content, regex matches).
    \item \( \mathsf{CD}_\ell \): \textbf{Control Dependencies} — Control-flow constructs affecting the execution of \( \ell \), such as conditional branches and loops.
    \item \( \mathsf{IC}_\ell \): \textbf{Invariant Constraints} — Semantic assumptions and correctness conditions that must be preserved before and after the patch (e.g., input format validity, crash avoidance).
    \item \( \mathsf{CG}_\ell \): \textbf{Call Graph Context} — A backward-traceable call chain showing which higher-level components transitively reach \( \ell \), capturing its functional embedding in the system.
\end{itemize}

For example, in the QDP parser issue described in Figure~\ref{fig:motivating}, the candidate patch modifies the `\_line\_type' function responsible for identifying command lines. The data dependencies include the regular expression `\_command\_re', which encodes the expected command syntax, and the input lines being matched against it. The control dependencies span the call chain from `Table.read', through `QDP.read', etc. % `_read_table_qdp`, `_get_tables_from_qdp_file`, and `_get_type_from_list_of_lines`, down to `_line_type`. 
The invariant constraints require that lowercase commands such as \texttt{read serr 1 2} be recognized as valid without breaking compatibility with existing uppercase-only behavior, and without introducing regressions or crashes elsewhere in the parsing process.

The patch context serves as a semantic scaffold for reasoning about the correctness and consistency of candidate patches, enabling principled refinement and post-hoc validation of learned edits.





% Understanding the issue alone is insufficient for generating robust patches—\ToolName{} must also capture how the code behaves in relation to the issue. This step builds a semantic model of the code’s intent, usage, and relevance to the bug.

% \textit{Execution Flow Extraction.} We extract high-level execution flows relevant to the issue and candidate patch, capturing how control or data moves through the code. In our motivating example, four flows were generated (\blackcircled{6}) —e.g., reading a QDP table , processing QDP lines, writing QDP tables, and regex operations—each representing a distinct pathway for localized repair.

% \textit{Step-Level Reasoning.} Each flow is decomposed into fine-grained, natural language steps (e.g., “read file line by line”, “extract header row”), which makes it easier to align reasoning with how developers typically conceptualize behavior. 
% To map steps to code, we prompt an LLM with step descriptions and file content. The model returns a structured JSON mapping semantic roles to code snippets, enabling precise, context-aware localization.




% To generate meaningful patches, it is not enough for an agent to understand what the issue is; it must also understand how the code operates in relation to that issue. This step involves building a semantic understanding of the code’s purpose, usage, and its connection to the issue, enabling more robust and context-aware repair of the code.

% \textit{Execution Flow Extraction}: We begin by identifying execution flows that are directly relevant to the issue and its corresponding patch. These flows represent high-level paths through the code that capture how data or control moves through specific functionalities. In the motivating example the relevant flow \blackcircled{6} describes the steps followed when using the QDP file to read a table. There were 3 other flows generated focused the steps relevant to processing QDP lines after reading a QDP table, the write functionality of the QDP table and the regex involved in the issue— each representing distinct paths that once fixed would ideally solve the issue and maintain consistency.

% By generating these flows, we isolate the minimal functional pathways needed to understand and fix the issue. This provides a structured lens through which the repair process can generate sematic aware code fixes.

% \textit{Step-Level Reasoning}: Each execution flow is further decomposed into a sequence of fine-grained, semantically meaningful steps. These steps correspond to atomic operations within the flow—such as reading a file line by line, extracting specific patterns, or applying conditional logic. Each step is expressed in natural language, which makes it easier to align reasoning with how developers typically conceptualize behavior.

% To map these semantic steps to actual code, we prompt an LLM with the step description and the content of the associated file. The model is tasked with returning a structured JSON output, where each key represents a semantic role (e.g., “extract header row”) and each value contains the corresponding code snippet. This allows for precise context localization with varying levels of granularity.

\subsubsection{Refining Patches}: 
After localizing code snippets for each step, \ToolName{} generates candidate patches using three inputs: the localized code, step-level semantics, and issue semantics (\circled{6}). This ensures that fixes are grounded in both the high-level intent and functional behavior, avoiding superficial or overfitted changes. The resulting patches are semantically rich, context-aware, and aligned with developer expectations. They are then passed to the reviewer agent.

In the motivating example, for the red-highlighted step in \blackcircled{6}, \ToolName{} identifies the ``\_get\_tables\_from\_qdp\_file'' function and correctly adjusts the case-sensitive comparison \texttt{v == "NO"} to a case-insensitive form, resolving the issue as shown in \blackcircled{2}. To reduce costs at this token-intensive stage, \ToolName{} supports optional caching (Appendix~\ref{appendix:cache}), retrieving previously generated fixes for repeated issue–patch pairs and storing new ones for future reuse.


% Once code snippets are localized for each step, we proceed to patch generation. At this stage, we give the LLM on three elements: the localized code, the semantics of the corresponding step, and the issue semantics obtained~\circled{6} in the earlier phase and generate candidate patches ensuring that the generated fixes are grounded in both the high-level intent of the issue and the functional behavior of the code. This approach enables semantically rich and context-aware patches. It avoids superficial or overfitted changes and instead yields repairs that align with both developer expectations and the underlying logic of the program. These patches are now sent to the reviewer agent. 

% In the motivating example, for the step highlighted in red in \blackcircled{6}, \ToolName{} accurately identifies the \_get\_tables\_from\_qdp\_file function as the relevant code snippet and correctly identifies that the v == "NO" comparison is important to resolve the issue and generates a patch that makes this comparison case-insensitive, as shown in \blackcircled{2}. This adjustment aligns the initial patch \blackcircled{3} with the intended issue semantics \blackcircled{5}, resulting in a consistent and semantically appropriate fix that resolves the issue.


% We also implement optional caching \ref{appendix:cache} at this stage solely to help reduce costs, as this is most token-intensive part of \ToolName{}'s workflow. The system checks for previous runs involving the same issue and initial patch, and if a match is found, it retrieves the previously generated fixes from the cache. Newly encountered issue–patch tuples are added to the cache, significantly reducing the cost of runs.

\subsection{Patch Reviewer Agent}
The final set of candidate patches is reviewed by an LLM-based reviewer agent (\circled{11}), which, given the issue description, determines patch relevance and provides justifications. Each patch is annotated with a boolean relevancy flag and an explanation, then passed to the final patch aggregation step. The reviewer agent uses a carefully designed prompt to align with the developer's intent and control the strictness of relevance assessment. This filtering step ensures only well-justified, semantically appropriate fixes are retained, increasing the likelihood of consistent and developer-aligned repairs.


% This final set of candidate patches are then passed to a reviewer agent \circled{11} which along with the original issue description is responsible for determining whether each patch is relevant or not along with an explanation supporting its decision. These explanations are appended to the corresponding patches and passed along to the final patching agent in the patch aggregation step, ensuring that only well-justified and contextually appropriate fixes are retained.

% The Reviewer Agent is implemented as an LLM-based module that takes in the issue and patch candidates and returns a structured JSON response containing a boolean relevancy flag and a textual justification for each patch. The prompt used by the Reviewer Agent is carefully crafted to capture the developer’s intent expressed in the issue description, and uses this understanding to guide patch selection and effectively control the level of strictness the LLM applies when determining patch relevance. This filtering step ensures that only those patches which truly satisfy the semantics and intent of the original issue are selected, increasing the likelihood of successful and developer-aligned repairs.

\subsection{Patch Aggregator}
The selected patches (\circled{12}) are passed to a Patch Aggregator (\circled{13}), which deduplicates and merges overlapping edits to ensure unique, non-conflicting fixes. These are combined with the initial patch (\circled{5}) and refined via an execution loop to produce the final patch (\circled{15}).

%\ray{check the following} 
Such an aggregator can be extended to a multi-agent setup where specialized agents generate complementary patches based on different kinds of semantics (see ablation: RQ2). The Patch Aggregator consolidates these diverse fixes into a coherent, validated patch that aligns with both the issue intent and code functionality.
% These selected patches \circled{12} are then sent to a Patch Aggregator \circled{13} that identifies and removes repeated patches and aggregates patches modifying similar lines of code ensuring unique patches with no overlap. Once this is done the patches are added along with the initial patch \circled{5} and refined using an execution loop to create the final patch \circled{15}.

\section{Multi-Approach Ensemble Selection -- \ToolName{}Multi}

Finally, the best patches (\circled{15}) from multiple ablations, are taken and fed to this module that uses an LLM as a judge with a high temperature to select the best patch over multiple iterations, the patch with the highest number of votes is then finally selected. \ToolName{}Multi runs 3 ablations of \ToolName{} - with all components, without the reviewer and without the repair stage. This varied ensemble approach leverages the strength of each approach and captures variance to select the absolute best patch.

==> samples/legacy/5_experiments.tex <==
\clearpage
\section{Experimental Setup}
\label{sec:experiments}
We address the following research questions:
\setlist{nolistsep}
\begin{itemize} [noitemsep,leftmargin=*]
\item \textbf{RQ1}: What is the impact of \ToolName{} on issue resolution?
\item \textbf{RQ2}: How useful are the individual components of \ToolName{} in patch generation?
\item \textbf{RQ3}: To what extent does incorporating Execution Semantics improve issue localization?

\CM{I did not understand the difference between RQ2 and RQ3, seems both of them are ablation study?}
\end{itemize}

\CM{cost of our agent, reproducility evaluation, backend LLM imapct, hyper-parameters sensitively}

\subsection{Evaluation Benchmark}
We evaluate \ToolName{} on SWEBench Lite~\cite{jimenez2024swebenchlanguagemodelsresolve}, a benchmark of 300 real-world GitHub issues across 11 Python repositories. For each issue, \ToolName{} receives the issue description and pre-fix codebase with regression tests, and outputs a single patch in git diff format, which is evaluated for successful resolution. \CM{I am not sure whether evaluating on only one dataset is convincing enough}




% We evaluate \ToolName{} on SWEBench Lite \cite{jimenez2024swebenchlanguagemodelsresolve} an evaluation framework that tests how well automated program repair systems resolve 300 real world github issues taken from 11 popular python repositories. For each issue the input given to \ToolName is the issue description along with the code base that contains pre-issue fix regression tests and gives a single patch in git diff format which is then tested on the evaluation framework to see if it successfully resolves the issue.




% \ToolName{} takes in the issue description and the corresponding code base along with the reproduction tests given by Amazon Q Developer \cite{AWSAmazonQDeveloper} that are preloaded and retrieved accordingly. These inputs then follow the workflow mentioned in the Figure(\ref{fig:pipeline}) and \ToolName{} generates a single patch per issue which is aggregated and evaluated on the benchmark. 

% \ToolName{} also strictly adheres to the SWE-bench guidelines and performs a single attempt per task instance (pass@1), does not use any SWE-bench test knowledge (e.g., PASS\_TO\_PASS or FAIL\_TO\_PASS), avoids the use of the hints field, and ensures that no web-browsing is used to retrieve SWE-bench solutions. All test patches generated by the model use only the available context and information and can be applied and run without error.

\subsection{Baseline}

To evaluate effectiveness, we compare \ToolName{} against SpecRover\cite{zhang2024autocoderoverautonomousprogramimprovement}, which forms our architectural baseline and reports 37\% accuracy on SWEBench Lite\footnote{\url{https://www.autocoderover.net/}}. 
%To evaluate the effectiveness of our approach, we use SpecRover as the baseline, as our method builds upon its core architecture. However, since the SWEBench leaderboard only reports the results for AutoCodeRover \cite{zhang2024autocoderoverautonomousprogramimprovement}, hence we use the numbers reported on SpecRovers \href{https://www.autocoderover.net/}{website} which indicates that it solved 37\% of SWEBench Lite issues. 
In addition to this we also compare against the best performing (as per SWEBench leaderboard) workflow based methods, Agentless \cite{xia2024agentlessdemystifyingllmbasedsoftware} and Agentic system OpenHands \cite{wang2024openhands}. 
%who's results are present in the SWEBench leaderboard.
We also include comparisons with other state-of-the-art APR methods, such as the agentic - CodeStory Aide, DARS Agent \cite{aggarwal2025dars}, and Globant Code Fixer Agent. These systems represent a range of workflow-based and agentic-based approaches, as well as a mix of open and closed-source implementations. This comprehensive comparison highlights the effectiveness and versatility of our method across diverse repair paradigms.

\subsection{Parameters}
\ToolName{} builds on workflow-based APR systems like SpecRover~\cite{ruan2024specrovercodeintentextraction}, reusing components for reproducer generation, context localization, and patching. We allow up to 3 pipeline retries, 15 localization rounds, and 10 reproducer attempts per issue, using Claude Sonnet 3.7 for its strong reasoning and code generation. To ensure stability, we fix the decoding temperature to zero and incorporate spectrum-based fault localization, improving reproducibility and reducing LLM-induced variance.


1. 


% \ToolName{} builds upon general workflow based automated program repair systems such as SpecRover \cite{ruan2024specrovercodeintentextraction}, from which we reuse key components such as reproducer generation, context localization, and patch generation. For each issue, we allow up to three overall retries across the pipeline, fifteen rounds of context localization, and ten rounds to generate a reproducer. For our experiments we use the latest Claude Sonnet 3.7 language model due to its superior reasoning and code generation capabilities. 

% %\subsection{Determinism and Randomness}
% To mitigate the inherently stochastic behavior of large language models, we set the decoding temperature to zero across all components and integrate spectrum-based fault localization  to enhance the stability and consistency of the localization phase. These measures collectively contribute to the reliability and reproducibility of \ToolName{}.


\subsection{Setup}
\ToolName{} takes as input the issue description, codebase, and preloaded Amazon Q Developer reproduction tests~\cite{AWSAmazonQDeveloper}, following the workflow in Figure~\ref{fig:pipeline} to generate one patch per issue for evaluation. \ToolName{} adheres strictly to SWE-bench guidelines: it performs a single pass@1 attempt, uses no test-specific metadata or hints, avoids web access, and ensures all patches are self-contained and executable within the provided context.

==> samples/legacy/6_results.tex <==
\clearpage

\section{Results}
\label{sec:results}

% \definecolor{lightmauve}{rgb}{0.86, 0.82, 1.0}

\subsection{RQ1: Impact on issue resolution}

%To show the impact of \ToolName{} on issue resolution we evaluate its efficacy in resolving 300 issues on SWEBench Lite, an evaluation framework that tests how well approaches can resolve real-world repository-level issues. We first show the performance of \ToolName{} on the benchmark, then show its improvement over the SpecRover baseline and finally compare it to other state of the art closed open source and closed source approaches. All reported results are taken from the SWEBench Lite online leaderboard except for our SpecRover baseline which we have re-run using a more powerful model Claude 3.7 over the reported baseline that uses Claude 3.5 for a more accurate comparison.

%\textit{\textbf{Result}}s: 
Table \ref{tab:results_of_models_on_swebench} shows the performance of various approaches on the SWEBench Lite benchmark. Our method, \ToolName{}, successfully resolves \textbf{151} issues, with a resolution rate of \textbf{50.33\%} and \MToolName{} resolves \textbf{155} issues, with a resolution rate of \textbf{51.66\%}. This represents a substantial improvement over the SpecRover baseline, outperforming it by \textbf{40} \& \textbf{44} additional resolved issues respectively with a \textbf{13.33} \& \textbf{14.67} percentage point increase in absolute resolution rate showing the effectiveness of incorporating issue and code semantics the program repair pipeline to improve performance.

\ToolName{} is the top purely workflow-based method and ranks second among all the open-source approaches on the SWEBench Lite leaderboard, behind only the agentic, fine-tuned DARS-Agent. Despite using only out-of-the-box models, \ToolName{} ranks 7th overall, highlighting the strength of incorporating code semantics in workflow methods. All results are from a single run.


% Our approach is the best approach that is purely workflow based and ranks second among all open-source methods on the leaderboard, surpassed only by DARS-Agent. This achievement is particularly noteworthy because, unlike DARS-Agent which leverages an agentic framework and a fine-tuned model, \ToolName{} employs a purely workflow based methodology with out of the box models. This distinction underscores the inherent strength and significant potential of workflow based techniques to push the boundaries of automated program repair. we acknowledge that while closed-source methods currently lead the field our approach still scores 8th place on the leaderboard and \ToolName{}'s strong performance relative to its baseline demonstrates the value derived from incorporating nuanced issue and code semantics in the repair process. We also note that these results are from a single run.
\ray{check}
Figure~\ref{fig:overlap} shows that our different design choices altogether can solve up to 154 issues. Thus, while extending our aggregator to a multi-agent (~\MToolName{}) setup, we could potentially solve up to 154 issues. 
The process can be further improved by smart sampling strategies, like Monte Carlo Tree sampling \cite{zhou2024languageagenttreesearch}. 


\textbf{Time and Costs}: Our approach takes on average 16 minutes to solve an issue and costs 6.9\$ dollars per issue when run on the parameters mentioned in the Setup section. These costs can be reduced to 4.77\$ an issue across multiple runs when using issue semantics and repair stage caching. We also note that the median cost per issue is 4.87\$ which is significantly lower then the average due to a few costly outliers such as scikit-14087 (>30\$) that skew the average cost.



% \begin{table*}[t]
%   \centering
%   \resizebox{.9\textwidth}{!}{
%   \begin{tabular}{l | c | c | c}
%     \hline
%     \textbf{Category} & \textbf{Approach} & \textbf{Open-Source} & \textbf{SWEBench Lite Performance} \\
%     \hline
%     Workflow-based & AutoCodeRover & Yes & 30.67 (92) \\
%     Workflow-based & SpecRover & Yes & 37\% (111) \\
%     Workflow-based & Agentless & Yes & 40.67\% (122) \\
%     Agentic & Openhands & Yes & 41.67\% (125) \\
%     Agentic & CodeStory Aide & No & 43\% (129) \\
%     \rowcolor{lightmauve} \textbf{Workflow-based} & \textbf{\ToolName{} + Claude 3.7 Sonnet} & \textbf{Yes} & \textbf{44.66\% (134)} \\
%     Agentic & DARS Agent & Yes & 47\% (141) \\
%     Agentic & Globant Code Fixer Agent & No & 48.33 \% (145) \\
%     \rowcolor{lightmauve} \textbf{Workflow-based} & \textbf{\ToolName{} + Gemini 2.5 Pro} & \textbf{Yes} & \textbf{50.33\% (151)} \\
%     \rowcolor{lightmauve} \textbf{Workflow-based} & \textbf{\MToolName{} + Claude 3.7 Sonnet} & \textbf{Yes} & \textbf{51.67\% (155)} \\
%   \hline
%   \end{tabular}
%   }
%   \caption{RQ1.~Efficacy of approaches on SWEBench Lite}
%   \label{tab:results_of_models_on_swebench}
% \end{table*}

\begin{table*}[t]
  \centering
  \resizebox{\textwidth}{!}{
  \begin{tabular}{l | l | c | l | c | c | c}
    \hline
    \textbf{Category} & \textbf{Approach} & \textbf{Open-Source} & \textbf{LLM} & \textbf{SWEBench Lite \% Resolved} & \textbf{Avg. Cost (\$)} & \textbf{Avg. Tokens} \\
    \hline
    Workflow-based & AutoCodeRover-v2 & Yes & GPT-4o & 30.67\% (92) & 0.65 & 37.6k \\
    Workflow-based & SpecRover & Yes & \NA & 37\% (111) & \NA & \NA \\
    Agentic & Moatless Tools & Yes & \claudeThreeFiveSonnet &  38.3\% (115) & 0.17 & \NA \\
    Workflow-based & Agentless-1.5 & Yes & \claudeThreeFiveSonnet & 40.67\% (122) & 1.12 & \NA \\
    Worklow-based & OrcaLoca + Agentless-1.5 & Yes & \claudeThreeFiveSonnet & 41\% (123) & \NA & \NA \\
    Agentic & Codart AI & No & \claudeThreeFiveSonnet & 41.67\% (125) & \NA & \NA \\
    Agentic & Openhands & Yes & CodeAct v2.1 & 41.67\% (125) & 2.14 & \NA \\
    Agentic & Lingxi & Yes & \NA & 42.67\% (126) & \NA & \NA \\
    Agentic & CodeStory Aide & No & \NA & 43\% (129) & \NA & \NA \\
    \rowcolor{lightmauve} \textbf{Workflow-based} & \textbf{\ToolName{}} & \textbf{Yes} & \textbf{\claudeThreeSevenSonnet} & \textbf{44.66\% (134)} & \textbf{6.9} & \textbf{1.11M} \\
    Agentic & DARS Agent & Yes & \claudeThreeFiveSonnet & 47\% (141) & 12.24 & \NA \\
    Agentic & devlo & No & \claudeThreeFiveSonnet & 47.33\% (142) & \NA & \NA \\
    Agentic & SWE-agent & Yes & \claudeThreeSevenSonnet & 48\% (144) & 1.62 & 521k \\
    Agentic & Globant Code Fixer Agent & No & \NA & 48.33\% (145) & \NA & \NA \\
    Agentic & ExpeRepair-v1.0 & Yes & \claudeThreeFiveSonnet + o3-mini & 48.33\% (145) & 2.07 & \NA \\
    Agentic & Gru & No & \NA & 48.67\% (146) & \NA & \NA \\
    Agentic & Codev & No & Claude 3.5 Haiku + Gemini 2.5 Flash/Pro + o4-mini & 49\% (147) & \NA & \NA \\
    Agentic & Blackbox AI Agent & No & \claudeThreeFiveSonnet & 49 \% (147) & \NA & \NA \\
    \rowcolor{lightmauve} \textbf{Workflow-based} & \textbf{\ToolName{}} & \textbf{Yes} & \textbf{\geminiTwoFivePro} & \textbf{50.33\% (151)} & \textbf{6.59} & \textbf{1.15M} \\
    \rowcolor{lightmauve} \textbf{Workflow-based} & \textbf{\MToolName{}} & \textbf{Yes} & \textbf{\claudeThreeSevenSonnet{} + \geminiTwoFivePro} & \textbf{51.67\% (155)} & \textbf{10.94} & \textbf{1.76M} \\
  \hline
  \end{tabular}
  }
  \caption{RQ1.~Efficacy of approaches on SWE-bench Lite with reported average cost and token consumption per task.}
  \label{tab:results_of_models_on_swebench_filled}
\end{table*}



%\subsection{RQ2: How useful are the individual components of \ToolName{} in patch generation?}
\subsection{RQ2: Ablation for patch generation}
\label{sec:rq2}

\ToolName{} consists of two main components: the Repair Stage (with Issue and Code Semantics) and the Reviewer Agent. We ablate four variants to assess their impact: (1) baseline with no components, (2) only the Repair Stage with both semantics, (3) Repair Stage with only Code Semantics (using the raw issue description), and (4) the full system with both semantics and the Reviewer Agent. Comparing (1) vs. (2) shows the value of semantics; (2) vs. (3) isolates the impact of issue semantics; (2) vs. (4) highlights the reviewer’s contribution. Execution semantics ablations are deferred to RQ3, as they target localization, not patch generation.



% The main components of \ToolName{} are the Repair stage and the Reviewer Agent with the Repair Stage incorporating Issue Semantics \& Code semantics. To show the impact of each we analyze the performance of four variations of \ToolName{} with and without certain components. (1) We look at the baseline performance of of \ToolName{} with no components, (2) The performance of \ToolName{} incorporating only the Repair Stage with Issue \& Code semantics, (3) The performance of \ToolName{} incorporating only the Repair Stage with Code semantics and not issue semantics - using the issue description in place of issue semantics and finally (4) \ToolName{} with all the components - a Repair Stage with issue and code semantics, along with the reviewer.

\begin{figure}
\centering
    \includegraphics[scale=0.6]{overlap_venn_diagram10.png}
    \caption[]{Overlap of Ablations - 161 issues resolved in total.}
    \label{fig:overlap}
\end{figure}

% \begin{table}[ht]
%   \centering
%   \begin{tabular}{lc}
%     \hline
%     \textbf{Approach} & \textbf{Solve Rate} \\
%     \hline
%     Baseline & 37\% (111)\\
%     w/ Repair Stage & 42\% (126) \\
%     \rowcolor{lightmauve} \textbf{w/ Repair Stage + Reviewer} & \textbf{43.33\% (130)} \\
%     \hline
%   \end{tabular}
%   \caption{Impact of Components on \ToolName{}Efficacy on SWEBench Lite} 
%   \label{tab:results_of_componenets}
% \end{table}

% \begin{table}[ht]
%   \centering
%   \begin{tabular}{lc}
%     \hline
%     \textbf{Approach} & \textbf{Solve Rate} \\
%     \hline
%     w/o Issue Semantics & 50\% (25) \\
%     \rowcolor{lightmauve} \textbf{w/ Issue Semantics} & \textbf{60\% (30)} \\
%     \hline
%   \end{tabular}
%   \caption{Impact of Issue Semantics on \ToolName{}Efficacy on a Random Set of 50 SWEBench Issues} 
%   \label{tab:results_of_issue_semantics}
% \end{table}

\begin{table*}[ht]
\parbox{.48\linewidth}{
\centering
\resizebox{\linewidth}{!} {
\begin{tabular}{lc}
    \hline
    \textbf{Approach w/ Claude 3.7 Sonnet} & \textbf{Solve Rate} \\
    \hline
    Baseline & 37\% (111)\\
    w/o Repair Stage & 40.33\% (121) \\
    w/ Repair Stage & 42\% (126) \\
    \rowcolor{lightmauve} \textbf{w/ Repair Stage + Reviewer} & \textbf{44.66\% (134)} \\
    \hline
  \end{tabular} 
  }
  \caption{RQ2.~Impact of Components on \ToolName{}Efficacy on SWEBench Lite} 
  \label{tab:results_of_componenets}
}
\hfill
\parbox{0.48\linewidth}{
\centering
%\resizebox{\linewidth}{!} {
\begin{tabular}{lc}
    \toprule
    \textbf{Approach w/ Claude 3.7 Sonnet} & \textbf{Solve Rate} \\
    \midrule
    w/o Issue Semantics & 50\% (25) \\
    \rowcolor{lightmauve} \textbf{w/ Issue Semantics} & \textbf{60\% (30)} \\
    \bottomrule
  \end{tabular}
 % }
  \caption{RQ2.~Impact of Issue Semantics on \ToolName{}Efficacy on a Random Set of 50 SWEBench Issues} 
  \label{tab:results_of_issue_semantics}
  }
\end{table*}

% Comparing (1) and (2) clearly shows the impact of incorporating semantics in resolving issues. Comparing (2) and (3) highlights how issue semantics contributes to performance, while comparing (2) and (4) isolates the effect of the reviewer agent. We leave ablations testing execution semantics to RQ3, as that component is designed to improve context localization rather than improve patch generation and validation.

Table \ref{tab:results_of_componenets} presents results from ablation (1) and ablation (3) with the mentioned Repair Stage using both types of semantics. Ablation (2), shown in Table 4, is run on a smaller subset of 50 issues and demonstrates the effect of using issue semantics vs just the issue~\ray{can we get baseline numbers on Table 3 50 examples?}.

\textit{\textbf{Results}}: Table \ref{tab:results_of_componenets} shows the initial improvement on the baseline when incorporating semantics increasing performance by 5\%. Further analysis of the newly resolved issues shows that \ToolName{} added complete fixes that complimented the patch in half of these issues leading to a successful resolution and in the other half of issues, the results provided by \ToolName{} solve the complete issue and during the final patch generation phase the suggestions from \ToolName{} lead to a complete resolution of the issue. However upon closer inspection of some of the failed patches, we see that \ToolName{}adds extra fixes that can potentially break existing functionality or go above and beyond a simple fix required to solve the issues. Such fixes are now filtered by the reviewer agent leading to a 2.66\% increase in performance giving us our best performing approach. These results validate the importance of the components in SemAgent's workflow.

Table \ref{tab:results_of_issue_semantics} evaluates the impact of incorporating issue semantics in the Repair Stage of \ToolName{}, using 49 randomly selected low-cost issues along with the motivating example. The results reveal that 5 issues remained unresolved when issue semantics were excluded. A closer analysis indicates that, in these cases, the LLM fails to produce meaningful modifications beyond the initially generated incorrect patch. Notably, in the motivating example, the absence of semantic context leads to inadequate handling of consistency and edge cases showing the critical role issue semantics play in \ToolName{}’s pipeline.

% \begin{table}[ht]
%   \centering
%   \begin{tabular}{lccc}
%     \hline
%     \textbf{Approach} & \textbf{Semantics} & \textbf{Reproducer} & \textbf{SWEBench Solve Rate} \\
%     \hline
%     (1) & ✗ & ✗ & 36\% \\
%     (2) & ✓ & ✗ & 41.67\% \\
%     (3) & ✓ & ✓ & 43.33\% \\
%     \hline
%   \end{tabular}
%   \caption{Results of \ToolName{} variants on SWEBench}
%   \label{tab:results_of_models_on_swebench}
% \end{table}



%\subsection{RQ3: To what extent does incorporating Execution Semantics improve issue localization?}


\input{samples/Results/rq3}

==> samples/legacy/implementation.tex <==


\subsection{Implementation Details}

\ToolName{}consists of 5 Modules - The execution semantics module, the typical program repair workflow module, the repair module, the reviewer module and the final aggregation module. In general we use greedy sampling and set the temperature as zero for more deterministic results, and run 3 pipeline retries for each issue that terminates early if a suitable patch is generated. We also use the initial patch as a "seed" that improves determinism and in caching to reduce redundant calls. It is also important to note that \ToolName{} takes as input the issue description, codebase, and preloaded Amazon Q Developer reproduction tests~\cite{AWSAmazonQDeveloper}, following the workflow in Figure~\ref{fig:pipeline} to generate one patch per issue for evaluation. \ToolName{} adheres strictly to SWE-bench guidelines: it performs a single pass@1 attempt, uses no test-specific metadata or hints, avoids web access, and ensures all patches are self-contained and executable within the provided context.

In the execution semantics stage, the initial generation of a reproducer is extended from AutoCodeRover, where an LLM is prompted to reason if a viable reproducer can be generated and proceeds based on the response. If the issue is reproducible then a reproducer workflow generation loop consisting of reproducer generation, LLM that validates it and re-iteration is run until a suitable reproducer is produced. We have appended this reproducer workflow with a refinement loop the uses an LLM as an advisor to refine and generate a reproducer with a more informative crash report, we then analyze the stack trace and rank suspicious files reverse ranked based on when the file was called (so the file called most closest to the crash is considered more suspicious) and filter based on if it exists in the buggy repo making sure we ignore irrelevant package calls. The execution semantics module also consists of an SBFL unit that runs SBFL on the buggy code base with the open sourced Amazon Q test patch added, this SBFL unit is also taken from AutoCodeRovers implementation and the top 5 suspicious files are then sent to the execution semantics module that takes in these 3 prongs - Enhanced crash report, and suspicious files from the stack trace and SBFL, this information is then reasoned on using an LLM and the results are added to the localization tool of AutoCodeRover for improved bug localization.

For the typical automated program repair workflow, \ToolName{}is modular enough that it is very easy to switch out the underlying program repair workflow used to generate a suitable initial patch and performs an initial localization of the issue. For our implementation we use SpecRover a sour underlying approach given the strong performance and extendability, this can theoretically be replace with any repair approach that generates an initial patch and localizes buggy files, also it is trivial to add the execution semantics information to most automated repair setups to improve localization, as most either use a variation of RAG or an agent iteratively finding the right file, in which case adding it in the prompt such as in AutoCodeRover leads to better performance. For our SWEBench Lite run \ToolName{}uses Claude 3.7 Sonnet a powerful model that balances performance and speed. We also use Gemini 2.5 Pro which performs exceedingly well on code related tasks. For SpecRover also cap the number of agent conversation rounds made during localization and api extraction from responses to 15 rounds as fewer then 8 rounds can lead to localization that is not fully fleshed out, and as the localization can end early if the LLM agrees that the correct file is localized, we do not waste too many LLM calls.

\TODO{This paragraph is some extra information, please move it to the right section accordingly -- } Since \ToolName{}is model agnostic so it is very easy to plug in different closed source models to reduce costs, our goal is to push the boundaries of what workflow based approaches are capable of so for our study we stick to powerful closed source models Claude 3.7 Sonnet and Gemini 2.5 Pro. We also acknowledge that LLMs will most likely get better and cheaper over time so it is imperative that \ToolName{}is made model agnostic.

For the program repair module, in the issue semantics phase the LLM is given the github issue and is given a prompt that explicitly converts a vague human given natural language issue into one where the intent is clear along with clear instructions on generalization and consistency in the code base along with clear instructions that an LLM agent would need to follow to actually implement the develops intent. For code semantics, the LLM is prompted to reason about data flows and data dependencies which we will refers to as "flows" that occur in the file that are relevant to the issue, and is guided to include the intermediate "steps" in each "flow". Next the LLM is iteratively given every step in each flow and maps the step to the relevant code - thereby aligning high-level execution-flow steps with concrete code snippets. Now the LLM is iteratively given each step and flow along with the mapped code snippets along with the issue semantics and is prompted to generated contextually aware fixes. Once all the fixes are generated, they are fed to an LLM that is prompted to combine them and remove repetitions to generate a final set of unique non-overlapping patches.

These patches are then sent to the reviewing module Where each fix is given to the LLM along with a prompt that asks it to give a score (relevant or not releavnt) along with the reasoning, the relevant fixes are then combine along with the reasoning and fed to the patch aggregator stage.

the patch aggregator builds on autocoderovers patch generation stage, where it takes in the initial seed patch, the reviewed fixes and performs a final edit validation refine loop where the validation consists of two signals, the result when applying the patch to the code base and running the reproducer to see if no exception arises, and also the regression tests with Amazon Q patches are run and the logs of the regression tests including the names of the failing tests and truncated run logs are sent to the agent to refine the patch and combine it properly, if at any point a patch is generated that can not be extracted into a git diff, then the patch generation is retried. Patch generation is capped at 3 iterations and the best patch is chosen, if none of the patches pass both the reproducer test and the regression tests then an LLM judge is used to select the best patch, if a patch passes both tests, then the most recent viable patch is chosen.

Finally the SemAgent Multi step is run. This component is designed to process a set of candidate patches generated from multiple parallel runs of SemAgent. The number of SemAgent configurations is adjustable, allowing for a trade-off between computational expense and potential performance gains. SemAgent Multi employs an iterative, LLM-based majority voting mechanism to identify the optimal patch. In this process, an LLM serves as a judge, evaluating the candidates over several cycles at a high temperature to ensure a thorough exploration of the solution space. The patch that secures the most votes is ultimately selected for final submission.

To ensure the LLM judge can make a highly informed decision, it is provided with comprehensive contextual information for each candidate patch. The inputs include:

\begin{itemize}
    \item The original faulty source codes and the corresponding files.
    \item The results from running regression tests with the applied patch along with the Amazon Q generated test git diff.
    \item The names and number of these failing tests.
\end{itemize}

The candidate patches are reverse-ranked based on the number of failing tests, allowing the LLM to prioritize solutions that are closer to being correct. This rich context with the faulty code and test feedback, enables the LLM to perform a nuanced evaluation that moves beyond simple pass/fail metrics since the existing regressions tests in the codebase may or may not accurately test the issue at hand and hence failing tests does not automatically mean that a patch is better or worse, instead we allow the LLM to analyze the failing tests and reason if the test failing is relevant or not.

For our evaluation, the candidate patches evaluated by SemAgent Multi are sourced from three distinct ablations of the core SemAgent pipeline:

\begin{itemize}
    \item A run without the repair stage.
    \item A run with the repair stage but without the reviewer component.
    \item The complete pipeline, including both the repair stage and the reviewer.
\end{itemize}

This strategy is designed to leverage the complementary strengths of these configurations, enabling SemAgent Multi to resolve a diverse spectrum of issues with varying complexity and nuance. By capturing the variance from different stages such as bug localization and patch generation, our approach aligns with state-of-the-art methods that utilize ensemble techniques. This multi-faceted model also acknowledges that simpler issues may not benefit from holistically superior but complex repairs, as minor changes to existing elements like return statements can cause regression test failures. SemAgent Multi is thus equipped to select a more targeted fix when it proves to be the most effective solution.

To identify the most effective configuration for our approach, we conducted a comprehensive series of ablation studies, systematically evaluating the impact of different components on the overall solve rate. These experiments focused on four key areas: the choice of the LLM judge, the use of a multi-LLM judging panel, the number of retry loops, and the temperature setting.

Our investigation into the LLM judge revealed that GPT 2.5 Pro was the top-performing model, achieving a solve rate of 155. This was a significant improvement over both Claude 3.7 and Claude 4, which recorded solve rates of 137 and 136, respectively. We also experimented with a multi-LLM setup that employed a majority vote among Claude 3.7, Claude 4, and GPT 2.5 Pro; however, this approach underperformed, yielding a solve rate of only 138 and it was found that since both claude 3.7 and 4 underperformed, the final patch selection also suffered as a result.

Further ablations focused on tuning the hyper parameters such as temperature and number of retry loops in the selection process. When varying the number of retry loops while using GPT 2.5 Pro as the judge and a temperature of 0.7 we observed a clear trend: performance improved with more iterations then plateaued as the number of retry loops crossed 5 retries. A single retry resulted in a solve rate of 145, which increased to 148 with three retries, and peaked at 155 with five retries. Similarly, adjusting the temperature proved critical. With five retries, a temperature of 0.7 achieved the highest score of 155, outperforming lower temperatures of 0.2 (148) and 0.0 (145), the combination of a higher temperature and large number of retry loops allows for better creativity and capturing variance.

Ultimately, these studies demonstrated that the optimal configuration consists of using GPT 2.5 Pro as the sole judge, combined with five retry loops and a temperature of 0.7 along with providing information of file contents and failing tests and providing an initial ranking accordingly.

% \begin{table*}[ht]
% \parbox{.48\linewidth}{
% \centering
% \resizebox{\linewidth}{!} {
% \begin{tabular}{lc}
%     \hline
%     \textbf{Approaches} & \textbf{Solve Rate} \\
%     \hline
%     LLM as judge:\\
%     Claude 4 Sonnet & 136 \\
%     Claude 3.7 Sonnet & 137 \\
%     GPT 2.5 Pro & 155 \\
%     Multi LLMs as judges w/ majority voting:\\
%     Claude 3.7,4 \& Gemini 2.5 Pro & 138\\
%     Varying num retry loops w/ GPT 2.5 Pro:\\
%     1 & 145\\
%     3 &  148\\
%     5 & 155\\
%     Varying temp with 5 retry loops w/ GPT 2.5 Pro:\\
%     0 & 145\\
%     0.2 & 148\\
%     0.7 & 155\\
    
%     \hline
%   \end{tabular} 
%   }
%   \caption{RQ2.~Impact of Components on \ToolName{}Efficacy on SWEBench Lite} 
%   \label{tab:results_of_semagent_multi}
% }
% \end{table*}

% For a professional look, ensure you have \usepackage{booktabs} in your LaTeX preamble.
% Also, define \ToolName, for example: \newcommand{\ToolName}{MyTool}

\begin{table*}[t]
  \centering
  \begin{tabular}{l | l | c}
    \hline
    \textbf{Component} & \textbf{Approach / Setting} & \textbf{SWEBench Lite Solve Rate} \\
    \hline
    LLM as Judge & Claude 3.7 & 45.67\% (137) \\
    LLM as Judge & Claude 4 & 46\% (138) \\
    \rowcolor{lightmauve} \textbf{LLM as Judge} & \textbf{GPT 2.5 Pro} & \textbf{51.67\%} (\textbf{155}) \\
    \hline
    Multi-LLM Judge & Claude 3.7, 4 \& GPT 2.5 Pro & 46.33\% (139) \\
    \hline
    Retry Loops & 1 Retry (w/ GPT 2.5 Pro, Temp 0.7) & 49\% (147) \\
    Retry Loops & 3 Retries (w/ GPT 2.5 Pro, Temp 0.7) & 50\% (150) \\
    \rowcolor{lightmauve} \textbf{Retry Loops} & \textbf{5 Retries (w/ GPT 2.5 Pro, Temp 0.7)} & \textbf{51.67\%} (\textbf{155}) \\
    \hline
    Temperature & Temp 0.0 (w/ GPT 2.5 Pro, 5 Retries) & 48.33\% (145) \\
    Temperature & Temp 0.2 (w/ GPT 2.5 Pro, 5 Retries) & 49.33\% (148) \\
    \rowcolor{lightmauve} \textbf{Temperature} & \textbf{Temp 0.7 (w/ GPT 2.5 Pro, 5 Retries)} & \textbf{51.67\%} (\textbf{155}) \\
    \hline
  \end{tabular}
  \caption{Ablation Study on \ToolName{}-Multi Components' Efficacy on SWE-Bench Lite.}
  \label{tab:ablation_study_swebench}
\end{table*}


% \ToolName{} builds on workflow-based APR systems like SpecRover~\cite{ruan2024specrovercodeintentextraction}, reusing components for reproducer generation, context localization, and patching. We allow up to 3 pipeline retries, 15 localization rounds, and 10 reproducer attempts per issue, using Claude Sonnet 3.7 for its strong reasoning and code generation. To ensure stability, we fix the decoding temperature to zero and incorporate spectrum-based fault localization, improving reproducibility and reducing LLM-induced variance.

==> samples/legacy/overview.tex <==


